Chase-escape in dynamic device-to-device networks

The present paper features results on global survival and extinction of an infection in a multi-layer network of mobile agents. Expanding on a model first presented in [CHJW22], we consider an urban environment, represented by line-segments in the plane, in which agents move according to a random waypoint model based on a Poisson point process. Whenever two agents are at sufficiently close proximity for a sufficiently long time the infection can be transmitted and then propagates into the system according to the same rule starting from a typical device. Inspired by wireless network architectures, the network is additionally equipped with a second class of agents that is able to transmit a patch to neighboring infected agents that in turn can further distribute the patch, leading to a chase-escape dynamics. We give conditions for parameter configurations that guarantee existence and absence of global survival as well as an in-and-out of the survival regime, depending on the speed of the devices. We also provide complementary results for the setting in which the chase-escape dynamics is defined as an independent process on the connectivity graph. The proofs mainly rest on percolation arguments via discretization and multiscale analysis.

==> Sec_PercResults.tex <==
We have described a multi-parameter connectivity network and the set of results presented in this report evolve around its clustering behavior. More precisely, we consider the associated random graph of connections up to time $T$
$$g_{\k,T,\g,\muv,\rho,r}(X^\la),$$
in which we will sometimes suppress the dependence on the street-system parameter $\gamma$, the time horizon $T$ as well as the mobility kernel $\kappa$, since we will often assume those parameters to be fixed. Recall that $g_{\muv,\rho,r}(X^\la)$ is the graph with vertices given by the Cox points in $X$ and in which any pair of Cox points is connected if  ~\ref{eq_connectedness} holds for at least one $t \in [0, T-\rho]$, i.e., their associated trajectories (described via $\k$ and $\muv$) are sufficiently close together (indicated by the parameter $r$) on the same street, for a sufficient amount of time (indicated by the parameter $\rho$). Let us highlight that, although the underlying mechanism for the edge-drawing depends on time, the graph $g_{\muv,\rho,r}(X^\la)$ is static, see also below for more comments. 


In view of the propagation of malware, or more generally any data, through the system, we start our analysis by considering percolation properties of $g_{\muv,\rho,r}(X^\la)$. That is, we say that the graph {\em percolates} if it contains an unbounded connected component. Here, percolation can be seen as a certain best-case scenario for the dissemination of data in the system. Indeed, our notion of percolation does not reflect that connections are in fact established at specific points in time, and that the actual path of a message through the dynamical network depends on when the message can hop from one device to another. In that sense, from the perspective of a message in the system, percolation assumes an optimal space-time placement of the connection events. In other words, in the absence of percolation, even an optimal space-time placement of the connection events will not lead to the possibility that data travels very far. 

Let us mention that a percolation analysis can additionally be motivated by assuming that the devices travel along their trajectory repeatedly (e.g., every day). Then, in case the handover of a message over multiple hops is impossible in one time window $[0,T]$, in the second iteration, when the possible transmissions in the first iteration are already performed, another set of transmissions will happen. 
Repeating this mechanism ultimately leads to a complete coverage of the connected component and then percolation indicates whether or not this component is large enough to support long-distance transmissions. 

To explain these motivations, let us make an example. Imagine three devices $X_1,X_2$ and $X_3$, where we see only a connection event at time $t_1\in [0,T]$ between $X_1$ and $X_2$ and another connection event at time $t_2\in [0,T]$ between $X_2$ and $X_3$. In our percolation picture, all three devices belong to the same connected component independent of the ordering of the times. However, if we entertain the idea that device $X_1$ sends a message to the devices in its component, in particular, to device $X_3$, then, in one time window this would require $t_1<t_2$, where then $X_2$ serves as a relay. Hence, in our first motivation, only in a connected component devices can exchange messages, however, we suppress the additional requirement that there also needs to be a sequence of connection events in the right order, in order to send messages in one time window. In our second motivation, which becomes relevant for example when dealing with malware, coming back to our example, even though $t_1<t_2$, in the first time window the malware can jump from $X_1$ to $X_2$ and then, in the second time window finally arrives at $X_3$. 


In view of percolation, we have the following scaling relations, where we also indicate now the dependence on $\k, T$ and $\gamma$. 
\begin{proposition}\label{prop_scale}
Let $\k, \muv$ and the parameters $T,\g,\la,\rho,r\ge 0$ be given. Then, for all $a>0$ we have that 
\begin{enumerate}
\item[(1)] $g_{\k[a],T,\g/a,\muv^a,\rho,ar}(X^{\la/a})$ percolates if and only if $g_{\k,T,\g,v,\rho,r}(X^\la)$ percolates and that
\item[(2)] $g_{\k,T/a,\g,\muv^a,\rho/a,r}(X^{\la})$ percolates if and only if $g_{\k,T,\g,v,\rho,r}(X^\la)$ percolates.
\end{enumerate}
\end{proposition}
\begin{proof}
If we scale the initial device positions (and the underlying street system) by a factor of $a$, then we see the same waypoint selection, if we also scale the waypoint kernels such that device $aX_i$ chooses position $aY_i$ on the street system $aS$ with the same probability as $X_i$ chooses $Y_i$ on $S$, leading to the kernel $\k[a]$. Note that the associated street and device densities are given by $\la/a$ and $\g/a$. Now, in order to see the same contact times, we also have to rescale the vicinity parameter $r$ by a factor $a$, and also rescale the speed by $a$. In particular, the time horizon as well as the connection times are not rescaled, since $a$ times the length traveled with $a$ times the speed leads to the same travel times. 

On the other hand, keeping the device position, streets and waypoint kernels fixed, while rescaling the speed by $a$, reproduced the percolation picture if we adjust the time horizon by a factor of $1/a$ and also the connection-time parameter accordingly by $1/a$. 
\end{proof}

Let us define the following critical parameters for percolation,
\begin{align*}
\Tc=\Tc(\k,\g,\la,\muv,\rho,r)&:=\inf\{\Tc>0\colon \P(g_{\k,T,\g,\muv,\rho,r}(X^\la)\text{ percolates})>0\}\\
\lac=\lac(\k,T,\g,\muv,\rho,r)&:=\inf\{\la>0\colon \P(g_{\k,T,\g,\muv,\rho,r}(X^\la)\text{ percolates})>0\}\\
\rhoc=\rhoc(\k,T,\g,\la,\muv,r)&:=\sup\{\rho>0\colon \P(g_{\k,T,\g,\muv,\rho,r}(X^\la)\text{ percolates})>0\}\\
\rc=\rc(\k,T,\g,\la,\muv,\rho)&:=\inf\{r>0\colon \P(g_{\k,T,\g,\muv,\rho,r}(X^\la)\text{ percolates})>0\}
\end{align*}
and note that these critical thresholds describe subcritical regimes in the sense that for $T<\Tc$, $\la<\lac$, $\rho>\rhoc$ or $r<\rc$, the system features percolation with probability zero. Further note that percolation is indeed monotone with respect to these parameters since longer time horizons, more devices, shorter connection-time thresholds and larger vicinity thresholds can only increase connectivity. Hence, our task is to investigate under what conditions we have that $0<\Tc,\lac,\rhoc,\rc<\infty$. 

Considering the dependence of percolation on the speed parameter $v$, the situation is substantially more complicated. Indeed, keeping all other parameters fixed and assuming for example a small density of devices, then, a slow speed does not allow any message to travel very far, and thus we expect to see absence of percolation. On the other hand, if the speed is large, then large gaps between devices can be bridged, but at the same time, the probability to be in close proximity for a sufficiently long time becomes very small, again leading to absence of percolation. In an intermediate speed regime in which also the other parameters allow for percolation, we then expect to see percolation with positive probability. 

Let us recall that we generally assume the support of $\muv$ to be contained in the minimal interval $[v_{\rm min},v_{\rm max}]$ with $0<v_{\rm min}\le v_{\rm max}<\infty$. 
Let us hence define two critical speed parameters
\begin{align*}
\vc=\vc(\k,T,\g,\la,\rho,r)&:=\inf\{v_{\rm max}>0\colon \P(g_{\k,T,\g,\muv,\rho,r}(X^\la)\text{ percolates})>0\}\\
\vcc=\vcc(\k,T,\g,\la,\rho,r)&:=\sup\{v_{\rm min}>0\colon \P(g_{\k,T,\g,\muv,\rho,r}(X^\la)\text{ percolates})>0\}
\end{align*}
and investigate settings in which $0<\vc<\vcc<\infty$.  

Let us start by investigating regimes where percolation is impossible.  

==> Sec_PercResults_NonPerc.tex <==
\subsection{Regimes for absence of percolation}
Our first result verifies that indeed, insufficiently many devices and a too slow speed lead to absence of percolation. 
\begin{theorem}\label{thm_lowintense}
For any $\k$ and all $\g,r,\rho\ge 0$ the following holds:
\begin{enumerate}
\item[(1)] For all $\la\ge 0$ and $\muv$ we have that $\Tc(\k,\g,\la,\muv,\rho,r)>0$,
\item[(2)] For all $T\ge 0$ and $\muv$ we have that $\lac(\k,T,\g,\muv,\rho,r)>0$ and 
\item[(3)] for all $T,\la\ge 0$ we have that $\vc(\k,T,\g,\la,\rho,r)>0$. 
\end{enumerate}
\end{theorem}
\begin{proof}
Each device can travel at most to a distance $Tv_{\rm max}$ from its starting position. Hence, any connected component of $g_{\k,T,\g,\muv,\rho,r}(X^\la)$ is contained in a connected component of the Gilbert graph $g_{2Tv_{\rm max}}(X^\la)$. In the Gilbert graph, any pair of points is connected if and only if their mutual distance is smaller than $2Tv$. But $g_{2Tv_{\rm max}}(X^\la)$ percolates with probability zero for all sufficiently small $T$, $v_{\rm max}$ or $\la$, see, for example~\cite{wias8}. 
\end{proof}

Let us mention that the comparison to the Gilbert graph, as described in the proof, allows us to derive first rough upper bounds for $\lac(\k,T,\g,\muv,\rho,r)$ and $\vc(\k,T,\g,\la,\rho,r)$ using the numerical analysis provided in earlier reports, for example~\cite{CRE1} and the associated research papers~\cite{wias9,wias8}. 

\medskip
Next, note that $\rc$ can very well be zero, since devices with non-parallel movement on a mutual edge share the same position exactly once for $r=0$. However, connections between devices that move together in the same direction can not exchange messages if $r=0$. For the consequences of this observation regarding the critical connectivity threshold, see Theorem~\ref{Thm_Rho_1} below. Let us note that, in principle, absence of percolation for $g_{\k,T,\g,\muv,\rho,0}(X^\la)$ could still imply $\rc(\k,T,\g,\la,\muv,\rho)=0$. This would be the case if $g_{\k,T,\g,\muv,\rho,r}(X^\la)$ percolates for all positive $r$, which indicates that the parameters $(\k,T,\g,\la,\muv,\rho,0)$ are critical for percolation, rendering a mathematical analysis extremely hard.

\medskip
In order to see absence of percolation for large speeds $v_{\rm min}$, first note that any street $s$ such that $2|s|/v_{\rm min}<\rho$ can not be used to exchange messages. However, every street can be used for traveling. More precisely, in order to establish a connection, any device has to remain at least a time of $\rho$ on some street and during that time travels at least a distance of $\rho v_{\rm min}$. As devices reverse their direction when they reach either their destination or their home, the minimal length of a street such that communication on it is possible is given by $\rho v_{\rm min}/2$. Although staying on a street of length smaller than $\rho v_{\rm min}/2$ is possible if both the initial position and the destination are on that street, those devices can only connect to the same type of devices that have both their home and destination on the same street. In that way, only local connective components are formed, we will ignore this possibility in the following considerations.

We have the following result on absence of percolation for sufficiently high speeds. 
\begin{theorem}\label{thm_largespeeds}
We consider street systems of Poisson--Voronoi or Poisson--Delaunay type, which are in particular exponentially stabilizing and asymptotically essentially connected.  
Then, for any $\k$ with bounded support and all $T,\g,\la,r\ge 0$ and all $\rho>0$ we have that $\vcc(\k,T,\g,\la,\rho,r)<\infty$. 
\end{theorem}
\begin{proof}[Idea for the proof]
Note that, as $v_{\rm min}$ tends to infinity, any device $X_i\in S$ eventually reaches its target location $Y_i\in S$ before time $T$.
In particular, it is very unlikely to see a path from $X_i$ to any of its possible target locations that reaches very far away from $X_i$ in $\R^2$, and these shortest paths can be determined independently of the device process. Additionally, only devices that have a sufficiently long street on a shortest path to at least one of their possible target locations can contribute to the connectivity, and again this can be determined independently of the device process. However, as $v$ tends to infinity, existence of these long streets becomes also unlikely, leading to a thinning of the devices and eventually to a subcritical regime. 

Formally, we dominate our percolation model by a subcritical {\em geostatistical Cox--Boolean model}, see also~\cite{AT17,SRPD04}, where the (random) environment determines both, the random radii associated to the points, and a sufficiently strong thinning of the Cox points. 

We present the complete proof in Section~\ref{Sec_Proof_Sub}.
\end{proof}

We still have to deal with the connection-time parameter $\rho$. For this, note that we have a trivial bound for the connection time, given by $\rhoc\le T/2$ since for $\rho> T/2$, in order to establish a connection on at least two different streets, the device has to stay on one street for at least $T/2$ time, leaving not enough time to form connections on any different street. Therefore, any device can only have connections to other devices that also spend the majority of their time on the same street.  As a consequence, each street forms its local connection cluster and communication between different clusters is impossible, which implies absence of percolation.
However, this trivial bound can be substantially improved, see below. Let us first make a statement on the absence of percolation for any positive $\rho$. 
\begin{theorem}\label{Thm_Rho_1}
For any $\k$ and all $T,\g,\la\ge 0$ we have that $\rhoc(\k,T,\g,\la,\muv,0)=0$.
\end{theorem}
\begin{proof}
As indicated above, connections between devices that move together in the same direction on a street, can not exchange messages if $r=0$. Additionally, if $r=0$, devices in non-parallel movement can never have a contact time that includes intervals of positive length, and hence $g_{\k,T,\g,\muv,\rho,0}(X^\la)$ does not percolate with positive probability for any $\rho>0$. 
\end{proof} 

In order to provide potentially better upper bounds for the critical connection time $\rhoc$ consider the following percolation model based on the street system. 
For all $S$ first denote by $S^{a}$ the thinned street system consisting of all streets in $S$ with length not smaller than $a\ge 0$. Second, we connect any pair of vertices that are endpoints of any of the long streets (with length not shorter than $a$) if and only if the length of the shortest path along the streets between them does not exceed $b\ge 0$. The resulting graph $S^{a,b}$ now consists of long streets and special edges between some of the endpoints of the long streets, see Figure~\ref{Fig_long_edge_percolation} for an illustration. 
\begin{figure}[h]
\centering
\input{Picture/pic6_long_edge_percolation_2.tex}
\caption{Realization of a street system given by a Poisson--Voronoi tessellation (red). Streets of length greater than $\rho v/2$ are drawn thick. Their endpoints (blue) are connected if their graph distance (indicated in dashed blue lines) is less than $v(T-2\rho)^+$. The blue vertices, combined with the thick red and thick blue edges form the percolation graph  $S^{v\rho/2,v(T-2\rho)^+}$.}
\label{Fig_long_edge_percolation}
\end{figure}
We say that $S^{a,b}$ percolates, if $S^{a,b}$ contains an infinitely-long component of connected streets and edges. Note that $\rho\mapsto \one\{S^{v_{\rm min}\rho/2,v_{\rm max}(T-2\rho)^+}\text{ percolates}\}$ is decreasing since we see less surviving streets and also less connections between endpoints of long streets. Here $(a)^+=\max\{a,0\}$. Hence, we can define a unique critical threshold via 
\begin{align*}
\rhoc'(T,\g,\muv)&:=\sup\{\rho>0\colon \P(S^{v_{\rm min}\rho/2,v_{\rm max}(T-2\rho)^+}\text{ percolates})>0\}.
\end{align*}
In principle we could have that $\rhoc'(T,\g,\muv)>T/2$ since $\P(S^{v_{\rm min}T/2,0}\text{ percolates})$ may be positive for sufficiently small $v_{\rm min}$, see Theorem~\ref{Thm_Rho_2} below for a related result. However, in this case, the reference model $S^{a,b}$ does not provide better bounds. We have the following theorem.
\begin{theorem}\label{Thm_Rho_1}
For any $\k$ and $\muv$ as well as all $T,\g,\la,r\ge 0$ we have that $\rhoc(\k,T,\g,\la,\muv,r)\le \min\{T/2,\rhoc'(T,\g,\muv)\}$.
\end{theorem}
Let us mention that $v\mapsto \one\{S^{v\rho/2,v(T-2\rho)^+}\text{ percolates}\}$ is not monotone since, for example, large velocities lead to more streets being eliminated, while also leading to the possibility to travel larger distances between remaining long streets.
Even for $T$ being much larger than $2\rho$, it is this interplay between the possibility to connect on sufficiently long streets and the ability to bridge between long streets (using all streets), that makes this percolation picture interesting. 
\begin{proof}
The central idea is that, even in a best-case scenario, where the device intensity is extremely large and the vicinity threshold is very small, in order for devices to form connections on at least two different streets, we must have that $2\rho+b/v\le T$, where $b$ is the graph distance between two endpoints of streets that are sufficiently long, and $v$ is a speed in the support of the speed distribution $\muv$. On the other hand, if every device can form a connection only on one single street, then the connected components in the original graph can only consist of either individual devices (that are unable to connect to any other device) or precisely those (finitely-many) devices associated to the street on which they form their connection. In particular, the initial position of a device does not have to lie on the street on which it establishes its connection. Hence, if $S^{v_{\rm min}\rho/2,v_{\rm max}(T-2\rho)^+}$ does not percolate, then also our system cannot percolate.
\end{proof} 

In order to complement Theorem~\ref{Thm_Rho_1}, as a final result for this section on absence of percolation, let us isolate a regime of fast speeds such that $\rhoc'(T,\g,\delta_v)<T/2$. Note that this is in general a nontrivial task since $v\mapsto \one\{S^{v\rho/2,v(T-2\rho)^+}\text{ percolates}\}$ is not monotone. Let us denote by 
\begin{align*}
a_{\rm c}(b,\g)&:=\sup\{a>0\colon \P(S^{a,b}\text{ percolates})>0\}
\end{align*}
the largest street-thinning parameter such that we see percolation with positive probability in the presence of additional edges between endpoints of long streets. 
We further write $a_{\rm c}(\g):=\lim_{b\downarrow0}a_{\rm c}(b,\g)$, where we note that the limit is in fact an infimum since $b\mapsto a_{\rm c}(b,\g)$ is decreasing. Then we have the following result. 
\begin{theorem}\label{Thm_Rho_2}
For any $\g>0$ we have $a_{\rm c}(\g)<\infty$. Further, for any $\k$, $T,\g,\la,r\ge 0$ and $v>4 a_{\rm c}(\g)/T$  it holds that $\rhoc'(T,\g,\delta_v)< T/2$.
\end{theorem}
In particular, the conditions presented in Theorem~\ref{Thm_Rho_2} imply that $\rhoc(\k,T,\g,\la,\delta_v,r)\le \rhoc'(T,\g,\delta_v)$ and analyzing absence of percolation for the auxiliary model  $S^{a,b}$ indeed provides better bounds. 
\begin{proof}
The proof for the finiteness of $a_{\rm c}(\g)$ rests on stabilization arguments and will be presented in Section~\ref{Sec_Proof_Sub_2}. 
Under the assumption that $a_{\rm c}(\g)<\infty$, note that, since $v>4 a_{\rm c}(\g)/T$, there exist $\eps,b>0$ such that $v(T/2-\eps)/2>a_{\rm c}(b,\g)$. In particular, we have that $\P(S^{v(T/2-\eps)/2,b'}\text{ percolates})=0$ for all $b'<b$. 
Hence, for $\rho>T/2-\eps$ and $\rho>T/2-b/(2v)$ we have also that $0=\P(S^{v\rho/2,v(T-2\rho)}\text{ percolates})$. 
Thus, $\rhoc'(T,\g,\delta_v)< T/2$, which finishes this part of the proof. 
\end{proof} 

==> Sec_PercResults_Perc.tex <==
\subsection{Regimes for percolation}
In order to see percolation we have a variety of parameters for possible adjustments. In view of Theorem~\ref{thm_lowintense}, note that for too small device intensity or speed, we can never see percolation. Hence, we assume the speed to be positive, i.e., $v_{\rm min}>0$ and naturally also the time horizon to be positive. In order to avoid complications coming from streets that are too short to support communications, in the first step, let us suppose that $\rho=0$ and prove existence of percolation for large device intensities. Let us present a condition for the waypoint kernel that relaxes isotropy around the starting position. 
We say that a kernel $\k$ is {\em $c$-well behaved} if for almost-all $S$ and all $x\in S$, if
\begin{align*}
B_c(x) \cap S \subset \text{supp}(\k^S(x, \d y)).
\end{align*}
Further, we say that $\k$ is {\em well behaved} if $\k$ is $c$-well behaved for some $c > 0$.
Let us note that both $\k'$ and $\k''$ are $R$-well behaved. 
Here is our first result for the immediate connectivity $\rho=0$. 
\begin{theorem}\label{thm_largeintense}
Let $\k$ be well behaved and translation-covariant. Then, for all $v_{\rm min},T,\g>0$ and $r\ge 0$ we have that $\lac(\k,T,\g,\muv,0,r)<\infty$. 
\end{theorem}
Let us mention that this statement is in fact true under the assumption that $\muv\neq\delta_0$, as can be seen from the proof. 

\begin{proof}[Idea for the proof]
In order to prove this theorem we will construct a coupling of the original process to an auxiliary process of open streets such that existence of an unbounded component of open streets implies percolation of the original model. Here, we say that a street is \textit{open} if devices on that street can connect to devices on all its neighboring streets and also inter-connect on that street. In particular, any infinite connected component of open streets contains an infinite connected component of devices. 
However, as $\la$ increases, the probability for a street to be open converges to one, resulting in a percolation regime for open streets. 
We present the complete proof in Section~\ref{Sec_Proof_Sup}. 
\end{proof}

We have now proved the existence of a percolation regime for $\rho = 0$, if $\lambda$ is sufficiently large. In order to move beyond this setting, note that for $\rho>0$, very short streets $s$ with $|s|<\rho v_{\rm min}/2$ can never be used to establish a connection, however, they can be used for traveling. 
As a consequence, for the case where $\rho > 0$ we need stronger assumptions on $\muv$ and $r$ in order to guarantee that $\lac(\k,T,\g,\muv,\rho,r)<\infty$.

Again, we want to compare our original model to a simpler model on the street system, which we describe now. For $a>0$ and $p \in (0,1]$ we denote by $S^{a,L,p}$ a street system generated by a two-step thinning procedure performed on $S$. That is, we eliminate each street in $S$ that has length less than $a$ or length larger than $L$. Afterwards, each remaining street is eliminated independently with probability $p$. 
We say that $S^{a,L,p}$ percolates, if it contains an infinite connected component of streets. Let us define a critical thinning parameter,
$$
a_{\rm c}(L,p,\g):=\sup\{a>0\colon \P(S^{a,L,p}\text{ percolates})>0\},
$$
and note that $L\mapsto a_{\rm c}(L,p,\g)$ is increasing where as $p\mapsto a_{\rm c}(L,p,\g)$ is decreasing. Hence, we can define $a_{\rm c}(\g):=\lim_{L\uparrow\infty,\, p\downarrow 0}a_{\rm c}(L,p,\g)$. In principle, $a_{\rm c}(\g)$ could very well be zero, however, in Theorem~\ref{thm_twicethinstreet} below, we show that indeed, $a_{\rm c}(\g)>0$ for all $\g>0$. 

With these definitions, we are in the position to state the following result.
\begin{theorem}\label{thm-percolation-rho-positive}
Let $\k$ be translation-covariant and $c$-well behaved for some $c>2\rho v_{\rm min}$. Further let $v_{\rm min},\g,\rho>0$, $r>\rho v_{\rm min}$ and $T>2\rho$. Then, if $2\rho v_{\rm min}<a_{\rm c}(\g)$, then $\lac(\k,T,\g,\muv,\rho,r)<\infty$.
\end{theorem}
Again, let us mention that the statement of the theorem is in fact true under the assumption that $\muv\neq\delta_0$, as can be seen from the proof. Let us further mention that in fact, in the proof, we derive an upper bound for $\lac$ given by some $\lac'(\k,\g,\muv,\rho,r)<\infty$ that is independent of $T$, as long as $T>2\rho$. This in particular implies that for $\la>\lac'(\k,\g,\muv,\rho,r)$  we have that $\Tc(\k,\g,\muv,\la,\rho,r)\le 2\rho<\infty$. 

\begin{proof}[Idea for the proof]
Similar to the proof of Theorem~\ref{thm_largeintense}, the main argument is a comparison of our model to a street system in which we thin out very short streets, very large streets and all individual streets independently. The thinning of short streets becomes necessary, since for positive $\rho$, short streets can never be used to establish connections. The independent thinning comes from the fact that, even for large device intensities, a street has good self-contained connectivity properties only with high probability. In order to get uniform control on this probability, we have to disregard very long streets. We present the complete proof in Section~\ref{Sec_Proof_Sup_2}. 
\end{proof}


The previous theorem heavily rests on the assumption that $S^{a, L, p}$ percolates. In the following theorem we will show that, indeed, there are regimes where it percolates. 
\begin{theorem}\label{thm_twicethinstreet}
For all asymptotically-essentially connected street system we have that $a_{\rm c}(\g)>0$. 
\end{theorem}
\begin{proof}[Idea for the proof]
The proof rests on a comparison with a finitely-dependent site percolation process on $\Z^2$, leveraging stabilization and asymptotic-essential-connectedness arguments. We present the complete proof in Section~\ref{Sec_Proof_Sup_3}. 
\end{proof}
